Anisotropic finite elements with high aspect ratio for an Asymptotic Preserving method for highly anisotropic elliptic equation

The concern of this work is the generalization of an Asymptotic Preserving method for the highly anisotropic elliptic equations presented in [P. Degond, A. Lozinski, J. Narski, and C. Negulescu. An asymptotic-preserving method for highly anisotropic elliptic equations based on a micro-macro decomposition. J. Comput. Phys., 231(7):2724{2740, 2012]. The limitations of the method introduced there in are omitted by the introduction of a stabilization term in the Asymptotic Reformulation. Furthermore, anisotropic error indicators and mesh adaptation algorithms are proposed and tested allowing to reduce considerably the number of mesh points required to achieve prescribed precision. Reported meshes have maximum aspect ratio greater than 500.

==> xfig/conc_profile.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(600,360)(0,0)
\font\gnuplot=cmr10 at 10pt
\gnuplot
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(60.0,40.0){\rule[-0.200pt]{125.027pt}{0.400pt}}
\put(579.0,40.0){\rule[-0.200pt]{0.400pt}{67.452pt}}
\put(60.0,320.0){\rule[-0.200pt]{125.027pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{67.452pt}}
\put(60,208){\usebox{\plotpoint}}
\multiput(60.00,208.59)(7.389,0.477){7}{\rule{5.460pt}{0.115pt}}
\multiput(60.00,207.17)(55.667,5.000){2}{\rule{2.730pt}{0.400pt}}
\multiput(127.00,213.59)(3.048,0.477){7}{\rule{2.340pt}{0.115pt}}
\multiput(127.00,212.17)(23.143,5.000){2}{\rule{1.170pt}{0.400pt}}
\put(155,217.67){\rule{1.204pt}{0.400pt}}
\multiput(155.00,217.17)(2.500,1.000){2}{\rule{0.602pt}{0.400pt}}
\multiput(160.00,219.60)(1.943,0.468){5}{\rule{1.500pt}{0.113pt}}
\multiput(160.00,218.17)(10.887,4.000){2}{\rule{0.750pt}{0.400pt}}
\multiput(174.00,223.60)(1.797,0.468){5}{\rule{1.400pt}{0.113pt}}
\multiput(174.00,222.17)(10.094,4.000){2}{\rule{0.700pt}{0.400pt}}
\put(187,227.17){\rule{0.900pt}{0.400pt}}
\multiput(187.00,226.17)(2.132,2.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(191.00,229.58)(1.069,0.491){17}{\rule{0.940pt}{0.118pt}}
\multiput(191.00,228.17)(19.049,10.000){2}{\rule{0.470pt}{0.400pt}}
\multiput(212.00,239.59)(0.762,0.482){9}{\rule{0.700pt}{0.116pt}}
\multiput(212.00,238.17)(7.547,6.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(221.00,245.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(221.00,244.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(234.00,254.59)(0.710,0.477){7}{\rule{0.660pt}{0.115pt}}
\multiput(234.00,253.17)(5.630,5.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(241.00,259.58)(0.554,0.495){33}{\rule{0.544pt}{0.119pt}}
\multiput(241.00,258.17)(18.870,18.000){2}{\rule{0.272pt}{0.400pt}}
\put(261,276.67){\rule{0.482pt}{0.400pt}}
\multiput(261.00,276.17)(1.000,1.000){2}{\rule{0.241pt}{0.400pt}}
\multiput(263.00,278.61)(0.462,0.447){3}{\rule{0.500pt}{0.108pt}}
\multiput(263.00,277.17)(1.962,3.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(266.00,281.60)(0.481,0.468){5}{\rule{0.500pt}{0.113pt}}
\multiput(266.00,280.17)(2.962,4.000){2}{\rule{0.250pt}{0.400pt}}
\put(270,284.67){\rule{0.482pt}{0.400pt}}
\multiput(270.00,284.17)(1.000,1.000){2}{\rule{0.241pt}{0.400pt}}
\put(272,286.17){\rule{0.482pt}{0.400pt}}
\multiput(272.00,285.17)(1.000,2.000){2}{\rule{0.241pt}{0.400pt}}
\put(274,287.67){\rule{0.482pt}{0.400pt}}
\multiput(274.00,287.17)(1.000,1.000){2}{\rule{0.241pt}{0.400pt}}
\put(276,287.67){\rule{0.241pt}{0.400pt}}
\multiput(276.00,288.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(277,285.67){\rule{0.241pt}{0.400pt}}
\multiput(277.00,286.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(277.0,287.0){\usebox{\plotpoint}}
\put(277.67,251){\rule{0.400pt}{3.373pt}}
\multiput(277.17,258.00)(1.000,-7.000){2}{\rule{0.400pt}{1.686pt}}
\put(278.0,265.0){\rule[-0.200pt]{0.400pt}{5.059pt}}
\put(278.67,153){\rule{0.400pt}{5.300pt}}
\multiput(278.17,164.00)(1.000,-11.000){2}{\rule{0.400pt}{2.650pt}}
\put(279.0,175.0){\rule[-0.200pt]{0.400pt}{18.308pt}}
\put(279.67,101){\rule{0.400pt}{1.445pt}}
\multiput(279.17,104.00)(1.000,-3.000){2}{\rule{0.400pt}{0.723pt}}
\put(280.0,107.0){\rule[-0.200pt]{0.400pt}{11.081pt}}
\put(280.67,91){\rule{0.400pt}{0.723pt}}
\multiput(280.17,92.50)(1.000,-1.500){2}{\rule{0.400pt}{0.361pt}}
\put(282,89.67){\rule{0.241pt}{0.400pt}}
\multiput(282.00,90.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(281.0,94.0){\rule[-0.200pt]{0.400pt}{1.686pt}}
\put(285,88.67){\rule{0.723pt}{0.400pt}}
\multiput(285.00,89.17)(1.500,-1.000){2}{\rule{0.361pt}{0.400pt}}
\put(283.0,90.0){\rule[-0.200pt]{0.482pt}{0.400pt}}
\put(291,87.17){\rule{6.300pt}{0.400pt}}
\multiput(291.00,88.17)(17.924,-2.000){2}{\rule{3.150pt}{0.400pt}}
\put(322,87.17){\rule{5.700pt}{0.400pt}}
\multiput(322.00,86.17)(16.169,2.000){2}{\rule{2.850pt}{0.400pt}}
\put(288.0,89.0){\rule[-0.200pt]{0.723pt}{0.400pt}}
\put(359,88.67){\rule{0.723pt}{0.400pt}}
\multiput(359.00,88.17)(1.500,1.000){2}{\rule{0.361pt}{0.400pt}}
\put(350.0,89.0){\rule[-0.200pt]{2.168pt}{0.400pt}}
\put(362,90){\usebox{\plotpoint}}
\put(362.67,90){\rule{0.400pt}{0.482pt}}
\multiput(362.17,90.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\put(362.0,90.0){\usebox{\plotpoint}}
\put(364,92){\usebox{\plotpoint}}
\put(364,92){\usebox{\plotpoint}}
\put(363.67,104){\rule{0.400pt}{1.686pt}}
\multiput(363.17,104.00)(1.000,3.500){2}{\rule{0.400pt}{0.843pt}}
\put(364.0,92.0){\rule[-0.200pt]{0.400pt}{2.891pt}}
\put(364.67,174){\rule{0.400pt}{4.336pt}}
\multiput(364.17,174.00)(1.000,9.000){2}{\rule{0.400pt}{2.168pt}}
\put(365.0,111.0){\rule[-0.200pt]{0.400pt}{15.177pt}}
\put(365.67,263){\rule{0.400pt}{1.686pt}}
\multiput(365.17,263.00)(1.000,3.500){2}{\rule{0.400pt}{0.843pt}}
\put(366.0,192.0){\rule[-0.200pt]{0.400pt}{17.104pt}}
\put(367,286.67){\rule{0.241pt}{0.400pt}}
\multiput(367.00,286.17)(0.500,1.000){2}{\rule{0.120pt}{0.400pt}}
\put(367.0,270.0){\rule[-0.200pt]{0.400pt}{4.095pt}}
\put(368,288){\usebox{\plotpoint}}
\put(370,286.17){\rule{0.700pt}{0.400pt}}
\multiput(370.00,287.17)(1.547,-2.000){2}{\rule{0.350pt}{0.400pt}}
\put(373,284.17){\rule{0.482pt}{0.400pt}}
\multiput(373.00,285.17)(1.000,-2.000){2}{\rule{0.241pt}{0.400pt}}
\multiput(375.00,282.93)(0.599,-0.477){7}{\rule{0.580pt}{0.115pt}}
\multiput(375.00,283.17)(4.796,-5.000){2}{\rule{0.290pt}{0.400pt}}
\multiput(381.00,277.92)(0.497,-0.494){27}{\rule{0.500pt}{0.119pt}}
\multiput(381.00,278.17)(13.962,-15.000){2}{\rule{0.250pt}{0.400pt}}
\put(368.0,288.0){\rule[-0.200pt]{0.482pt}{0.400pt}}
\put(396.0,264.0){\usebox{\plotpoint}}
\put(397,261.17){\rule{0.900pt}{0.400pt}}
\multiput(397.00,262.17)(2.132,-2.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(401.00,259.92)(0.696,-0.495){33}{\rule{0.656pt}{0.119pt}}
\multiput(401.00,260.17)(23.639,-18.000){2}{\rule{0.328pt}{0.400pt}}
\put(426,241.17){\rule{0.700pt}{0.400pt}}
\multiput(426.00,242.17)(1.547,-2.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(429.00,239.92)(1.158,-0.494){25}{\rule{1.014pt}{0.119pt}}
\multiput(429.00,240.17)(29.895,-14.000){2}{\rule{0.507pt}{0.400pt}}
\multiput(461.00,225.94)(1.943,-0.468){5}{\rule{1.500pt}{0.113pt}}
\multiput(461.00,226.17)(10.887,-4.000){2}{\rule{0.750pt}{0.400pt}}
\multiput(475.00,221.93)(1.834,-0.489){15}{\rule{1.522pt}{0.118pt}}
\multiput(475.00,222.17)(28.841,-9.000){2}{\rule{0.761pt}{0.400pt}}
\multiput(507.00,212.93)(4.606,-0.477){7}{\rule{3.460pt}{0.115pt}}
\multiput(507.00,213.17)(34.819,-5.000){2}{\rule{1.730pt}{0.400pt}}
\put(397.0,263.0){\usebox{\plotpoint}}
\put(550,207.67){\rule{6.986pt}{0.400pt}}
\multiput(550.00,208.17)(14.500,-1.000){2}{\rule{3.493pt}{0.400pt}}
\put(549.0,209.0){\usebox{\plotpoint}}
\end{picture}


==> xfig/phase_profile.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(600,360)(0,0)
\font\gnuplot=cmr10 at 10pt
\gnuplot
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(60.0,40.0){\rule[-0.200pt]{125.027pt}{0.400pt}}
\put(579.0,40.0){\rule[-0.200pt]{0.400pt}{67.452pt}}
\put(60.0,320.0){\rule[-0.200pt]{125.027pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{67.452pt}}
\put(60,63){\usebox{\plotpoint}}
\put(274,62.67){\rule{0.482pt}{0.400pt}}
\multiput(274.00,62.17)(1.000,1.000){2}{\rule{0.241pt}{0.400pt}}
\put(60.0,63.0){\rule[-0.200pt]{51.553pt}{0.400pt}}
\put(276.0,64.0){\usebox{\plotpoint}}
\put(276.67,66){\rule{0.400pt}{0.482pt}}
\multiput(276.17,66.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\put(277.0,64.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(277.67,93){\rule{0.400pt}{4.095pt}}
\multiput(277.17,93.00)(1.000,8.500){2}{\rule{0.400pt}{2.048pt}}
\put(278.0,68.0){\rule[-0.200pt]{0.400pt}{6.022pt}}
\put(278.67,199){\rule{0.400pt}{6.263pt}}
\multiput(278.17,199.00)(1.000,13.000){2}{\rule{0.400pt}{3.132pt}}
\put(279.0,110.0){\rule[-0.200pt]{0.400pt}{21.440pt}}
\put(279.67,277){\rule{0.400pt}{1.927pt}}
\multiput(279.17,277.00)(1.000,4.000){2}{\rule{0.400pt}{0.964pt}}
\put(280.0,225.0){\rule[-0.200pt]{0.400pt}{12.527pt}}
\put(280.67,293){\rule{0.400pt}{0.482pt}}
\multiput(280.17,293.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\put(281.67,295){\rule{0.400pt}{0.482pt}}
\multiput(281.17,295.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\put(281.0,285.0){\rule[-0.200pt]{0.400pt}{1.927pt}}
\put(362,295.67){\rule{0.241pt}{0.400pt}}
\multiput(362.00,296.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(362.67,294){\rule{0.400pt}{0.482pt}}
\multiput(362.17,295.00)(1.000,-1.000){2}{\rule{0.400pt}{0.241pt}}
\put(283.0,297.0){\rule[-0.200pt]{19.031pt}{0.400pt}}
\put(364,294){\usebox{\plotpoint}}
\put(364,294){\usebox{\plotpoint}}
\put(363.67,273){\rule{0.400pt}{1.927pt}}
\multiput(363.17,277.00)(1.000,-4.000){2}{\rule{0.400pt}{0.964pt}}
\put(364.0,281.0){\rule[-0.200pt]{0.400pt}{3.132pt}}
\put(364.67,179){\rule{0.400pt}{5.300pt}}
\multiput(364.17,190.00)(1.000,-11.000){2}{\rule{0.400pt}{2.650pt}}
\put(365.0,201.0){\rule[-0.200pt]{0.400pt}{17.345pt}}
\put(365.67,87){\rule{0.400pt}{2.168pt}}
\multiput(365.17,91.50)(1.000,-4.500){2}{\rule{0.400pt}{1.084pt}}
\put(366.0,96.0){\rule[-0.200pt]{0.400pt}{19.995pt}}
\put(366.67,64){\rule{0.400pt}{0.482pt}}
\multiput(366.17,65.00)(1.000,-1.000){2}{\rule{0.400pt}{0.241pt}}
\put(367.0,66.0){\rule[-0.200pt]{0.400pt}{5.059pt}}
\put(368,64){\usebox{\plotpoint}}
\put(368,62.67){\rule{0.482pt}{0.400pt}}
\multiput(368.00,63.17)(1.000,-1.000){2}{\rule{0.241pt}{0.400pt}}
\put(370.0,63.0){\rule[-0.200pt]{50.348pt}{0.400pt}}
\end{picture}


==> xfig/profile-concentration.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(60.0,40.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(1439.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60.0,860.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60,535){\usebox{\plotpoint}}
\multiput(60.00,535.58)(4.809,0.495){33}{\rule{3.878pt}{0.119pt}}
\multiput(60.00,534.17)(161.951,18.000){2}{\rule{1.939pt}{0.400pt}}
\multiput(234.00,553.58)(1.812,0.497){51}{\rule{1.537pt}{0.120pt}}
\multiput(234.00,552.17)(93.810,27.000){2}{\rule{0.769pt}{0.400pt}}
\multiput(331.00,580.59)(1.255,0.485){11}{\rule{1.071pt}{0.117pt}}
\multiput(331.00,579.17)(14.776,7.000){2}{\rule{0.536pt}{0.400pt}}
\multiput(348.00,587.58)(0.791,0.494){25}{\rule{0.729pt}{0.119pt}}
\multiput(348.00,586.17)(20.488,14.000){2}{\rule{0.364pt}{0.400pt}}
\multiput(370.00,601.58)(0.782,0.497){47}{\rule{0.724pt}{0.120pt}}
\multiput(370.00,600.17)(37.497,25.000){2}{\rule{0.362pt}{0.400pt}}
\multiput(409.00,626.58)(0.561,0.494){29}{\rule{0.550pt}{0.119pt}}
\multiput(409.00,625.17)(16.858,16.000){2}{\rule{0.275pt}{0.400pt}}
\multiput(427.00,642.58)(0.567,0.498){71}{\rule{0.554pt}{0.120pt}}
\multiput(427.00,641.17)(40.850,37.000){2}{\rule{0.277pt}{0.400pt}}
\multiput(469.00,679.59)(0.560,0.488){13}{\rule{0.550pt}{0.117pt}}
\multiput(469.00,678.17)(7.858,8.000){2}{\rule{0.275pt}{0.400pt}}
\multiput(478.58,687.00)(0.498,0.526){73}{\rule{0.120pt}{0.521pt}}
\multiput(477.17,687.00)(38.000,38.919){2}{\rule{0.400pt}{0.261pt}}
\multiput(516.00,727.58)(0.534,0.494){25}{\rule{0.529pt}{0.119pt}}
\multiput(516.00,726.17)(13.903,14.000){2}{\rule{0.264pt}{0.400pt}}
\multiput(531.00,741.58)(0.713,0.495){35}{\rule{0.668pt}{0.119pt}}
\multiput(531.00,740.17)(25.613,19.000){2}{\rule{0.334pt}{0.400pt}}
\multiput(558.00,760.59)(0.560,0.488){13}{\rule{0.550pt}{0.117pt}}
\multiput(558.00,759.17)(7.858,8.000){2}{\rule{0.275pt}{0.400pt}}
\multiput(567.00,768.58)(0.964,0.491){17}{\rule{0.860pt}{0.118pt}}
\multiput(567.00,767.17)(17.215,10.000){2}{\rule{0.430pt}{0.400pt}}
\multiput(586.00,778.61)(1.355,0.447){3}{\rule{1.033pt}{0.108pt}}
\multiput(586.00,777.17)(4.855,3.000){2}{\rule{0.517pt}{0.400pt}}
\put(593,780.67){\rule{0.241pt}{0.400pt}}
\multiput(593.00,780.17)(0.500,1.000){2}{\rule{0.120pt}{0.400pt}}
\put(594,782.17){\rule{0.900pt}{0.400pt}}
\multiput(594.00,781.17)(2.132,2.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(598.00,784.59)(1.304,0.482){9}{\rule{1.100pt}{0.116pt}}
\multiput(598.00,783.17)(12.717,6.000){2}{\rule{0.550pt}{0.400pt}}
\put(613,790.17){\rule{1.100pt}{0.400pt}}
\multiput(613.00,789.17)(2.717,2.000){2}{\rule{0.550pt}{0.400pt}}
\put(230.0,553.0){\rule[-0.200pt]{0.964pt}{0.400pt}}
\put(619.17,787){\rule{0.400pt}{1.100pt}}
\multiput(618.17,789.72)(2.000,-2.717){2}{\rule{0.400pt}{0.550pt}}
\put(618.0,792.0){\usebox{\plotpoint}}
\put(621,787){\usebox{\plotpoint}}
\put(621.17,771){\rule{0.400pt}{3.100pt}}
\multiput(620.17,779.57)(2.000,-8.566){2}{\rule{0.400pt}{1.550pt}}
\put(621.0,786.0){\usebox{\plotpoint}}
\put(622.67,730){\rule{0.400pt}{5.059pt}}
\multiput(622.17,740.50)(1.000,-10.500){2}{\rule{0.400pt}{2.529pt}}
\put(623.0,751.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(623.67,687){\rule{0.400pt}{5.059pt}}
\multiput(623.17,697.50)(1.000,-10.500){2}{\rule{0.400pt}{2.529pt}}
\put(624.0,708.0){\rule[-0.200pt]{0.400pt}{5.300pt}}
\put(624.67,588){\rule{0.400pt}{7.468pt}}
\multiput(624.17,603.50)(1.000,-15.500){2}{\rule{0.400pt}{3.734pt}}
\put(625.0,619.0){\rule[-0.200pt]{0.400pt}{16.381pt}}
\put(625.67,485){\rule{0.400pt}{7.950pt}}
\multiput(625.17,501.50)(1.000,-16.500){2}{\rule{0.400pt}{3.975pt}}
\put(626.0,518.0){\rule[-0.200pt]{0.400pt}{16.863pt}}
\put(626.67,353){\rule{0.400pt}{8.432pt}}
\multiput(626.17,370.50)(1.000,-17.500){2}{\rule{0.400pt}{4.216pt}}
\put(627.0,388.0){\rule[-0.200pt]{0.400pt}{23.367pt}}
\put(627.67,235){\rule{0.400pt}{6.263pt}}
\multiput(627.17,248.00)(1.000,-13.000){2}{\rule{0.400pt}{3.132pt}}
\put(628.0,261.0){\rule[-0.200pt]{0.400pt}{22.163pt}}
\put(628.67,184){\rule{0.400pt}{3.614pt}}
\multiput(628.17,191.50)(1.000,-7.500){2}{\rule{0.400pt}{1.807pt}}
\put(629.0,199.0){\rule[-0.200pt]{0.400pt}{8.672pt}}
\put(629.67,157){\rule{0.400pt}{1.686pt}}
\multiput(629.17,160.50)(1.000,-3.500){2}{\rule{0.400pt}{0.843pt}}
\put(630.0,164.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(630.67,138){\rule{0.400pt}{1.686pt}}
\multiput(630.17,141.50)(1.000,-3.500){2}{\rule{0.400pt}{0.843pt}}
\put(631.0,145.0){\rule[-0.200pt]{0.400pt}{2.891pt}}
\put(632.17,132){\rule{0.400pt}{0.900pt}}
\multiput(631.17,134.13)(2.000,-2.132){2}{\rule{0.400pt}{0.450pt}}
\put(632.0,136.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(634,132){\usebox{\plotpoint}}
\put(634,130.17){\rule{0.700pt}{0.400pt}}
\multiput(634.00,131.17)(1.547,-2.000){2}{\rule{0.350pt}{0.400pt}}
\put(642,128.67){\rule{0.964pt}{0.400pt}}
\multiput(642.00,129.17)(2.000,-1.000){2}{\rule{0.482pt}{0.400pt}}
\put(646,127.67){\rule{1.204pt}{0.400pt}}
\multiput(646.00,128.17)(2.500,-1.000){2}{\rule{0.602pt}{0.400pt}}
\multiput(651.00,126.93)(7.434,-0.485){11}{\rule{5.700pt}{0.117pt}}
\multiput(651.00,127.17)(86.169,-7.000){2}{\rule{2.850pt}{0.400pt}}
\put(637.0,130.0){\rule[-0.200pt]{1.204pt}{0.400pt}}
\put(749,121){\usebox{\plotpoint}}
\multiput(749.00,121.59)(8.614,0.477){7}{\rule{6.340pt}{0.115pt}}
\multiput(749.00,120.17)(64.841,5.000){2}{\rule{3.170pt}{0.400pt}}
\put(827,125.67){\rule{6.023pt}{0.400pt}}
\multiput(827.00,125.17)(12.500,1.000){2}{\rule{3.011pt}{0.400pt}}
\put(852,126.67){\rule{1.686pt}{0.400pt}}
\multiput(852.00,126.17)(3.500,1.000){2}{\rule{0.843pt}{0.400pt}}
\put(859,127.67){\rule{0.964pt}{0.400pt}}
\multiput(859.00,127.17)(2.000,1.000){2}{\rule{0.482pt}{0.400pt}}
\put(866,128.67){\rule{0.241pt}{0.400pt}}
\multiput(866.00,128.17)(0.500,1.000){2}{\rule{0.120pt}{0.400pt}}
\put(863.0,129.0){\rule[-0.200pt]{0.723pt}{0.400pt}}
\put(867.67,130){\rule{0.400pt}{0.723pt}}
\multiput(867.17,130.00)(1.000,1.500){2}{\rule{0.400pt}{0.361pt}}
\put(867.0,130.0){\usebox{\plotpoint}}
\put(869.0,133.0){\usebox{\plotpoint}}
\put(869.67,138){\rule{0.400pt}{1.204pt}}
\multiput(869.17,138.00)(1.000,2.500){2}{\rule{0.400pt}{0.602pt}}
\put(870.0,133.0){\rule[-0.200pt]{0.400pt}{1.204pt}}
\put(871,143){\usebox{\plotpoint}}
\put(870.67,145){\rule{0.400pt}{1.927pt}}
\multiput(870.17,145.00)(1.000,4.000){2}{\rule{0.400pt}{0.964pt}}
\put(871.0,143.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(871.67,171){\rule{0.400pt}{4.095pt}}
\multiput(871.17,171.00)(1.000,8.500){2}{\rule{0.400pt}{2.048pt}}
\put(872.0,153.0){\rule[-0.200pt]{0.400pt}{4.336pt}}
\put(873,188){\usebox{\plotpoint}}
\put(872.67,211){\rule{0.400pt}{4.818pt}}
\multiput(872.17,211.00)(1.000,10.000){2}{\rule{0.400pt}{2.409pt}}
\put(873.0,188.0){\rule[-0.200pt]{0.400pt}{5.541pt}}
\put(873.67,300){\rule{0.400pt}{6.023pt}}
\multiput(873.17,300.00)(1.000,12.500){2}{\rule{0.400pt}{3.011pt}}
\put(874.0,231.0){\rule[-0.200pt]{0.400pt}{16.622pt}}
\put(874.67,391){\rule{0.400pt}{11.081pt}}
\multiput(874.17,391.00)(1.000,23.000){2}{\rule{0.400pt}{5.541pt}}
\put(875.0,325.0){\rule[-0.200pt]{0.400pt}{15.899pt}}
\put(875.67,555){\rule{0.400pt}{7.227pt}}
\multiput(875.17,555.00)(1.000,15.000){2}{\rule{0.400pt}{3.613pt}}
\put(876.0,437.0){\rule[-0.200pt]{0.400pt}{28.426pt}}
\put(876.67,658){\rule{0.400pt}{2.650pt}}
\multiput(876.17,658.00)(1.000,5.500){2}{\rule{0.400pt}{1.325pt}}
\put(877.0,585.0){\rule[-0.200pt]{0.400pt}{17.586pt}}
\put(877.67,724){\rule{0.400pt}{3.854pt}}
\multiput(877.17,724.00)(1.000,8.000){2}{\rule{0.400pt}{1.927pt}}
\put(878.0,669.0){\rule[-0.200pt]{0.400pt}{13.249pt}}
\put(878.67,753){\rule{0.400pt}{3.614pt}}
\multiput(878.17,753.00)(1.000,7.500){2}{\rule{0.400pt}{1.807pt}}
\put(879.0,740.0){\rule[-0.200pt]{0.400pt}{3.132pt}}
\put(879.67,774){\rule{0.400pt}{2.168pt}}
\multiput(879.17,774.00)(1.000,4.500){2}{\rule{0.400pt}{1.084pt}}
\put(880.0,768.0){\rule[-0.200pt]{0.400pt}{1.445pt}}
\put(881.17,785){\rule{0.400pt}{0.900pt}}
\multiput(880.17,785.00)(2.000,2.132){2}{\rule{0.400pt}{0.450pt}}
\put(881.0,783.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(883,788.67){\rule{0.964pt}{0.400pt}}
\multiput(883.00,789.17)(2.000,-1.000){2}{\rule{0.482pt}{0.400pt}}
\put(883.0,789.0){\usebox{\plotpoint}}
\put(888,787.67){\rule{0.241pt}{0.400pt}}
\multiput(888.00,788.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\multiput(889.00,786.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(889.00,787.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(903.00,780.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(903.00,781.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(918.00,771.92)(0.920,-0.492){19}{\rule{0.827pt}{0.118pt}}
\multiput(918.00,772.17)(18.283,-11.000){2}{\rule{0.414pt}{0.400pt}}
\multiput(938.00,760.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(938.00,761.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(952.00,749.92)(0.539,-0.498){73}{\rule{0.532pt}{0.120pt}}
\multiput(952.00,750.17)(39.897,-38.000){2}{\rule{0.266pt}{0.400pt}}
\multiput(993.59,710.72)(0.488,-0.560){13}{\rule{0.117pt}{0.550pt}}
\multiput(992.17,711.86)(8.000,-7.858){2}{\rule{0.400pt}{0.275pt}}
\multiput(1001.00,702.92)(0.540,-0.498){71}{\rule{0.532pt}{0.120pt}}
\multiput(1001.00,703.17)(38.895,-37.000){2}{\rule{0.266pt}{0.400pt}}
\multiput(1041.00,665.92)(0.575,-0.497){63}{\rule{0.561pt}{0.120pt}}
\multiput(1041.00,666.17)(36.836,-33.000){2}{\rule{0.280pt}{0.400pt}}
\multiput(1079.00,632.93)(0.599,-0.477){7}{\rule{0.580pt}{0.115pt}}
\multiput(1079.00,633.17)(4.796,-5.000){2}{\rule{0.290pt}{0.400pt}}
\multiput(1085.00,627.92)(0.778,-0.497){55}{\rule{0.721pt}{0.120pt}}
\multiput(1085.00,628.17)(43.504,-29.000){2}{\rule{0.360pt}{0.400pt}}
\multiput(1130.00,598.93)(0.710,-0.477){7}{\rule{0.660pt}{0.115pt}}
\multiput(1130.00,599.17)(5.630,-5.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(1137.00,593.92)(1.325,-0.497){57}{\rule{1.153pt}{0.120pt}}
\multiput(1137.00,594.17)(76.606,-30.000){2}{\rule{0.577pt}{0.400pt}}
\put(887.0,789.0){\usebox{\plotpoint}}
\put(1217,563.17){\rule{1.700pt}{0.400pt}}
\multiput(1217.00,564.17)(4.472,-2.000){2}{\rule{0.850pt}{0.400pt}}
\multiput(1225.00,561.93)(2.126,-0.489){15}{\rule{1.744pt}{0.118pt}}
\multiput(1225.00,562.17)(33.379,-9.000){2}{\rule{0.872pt}{0.400pt}}
\multiput(1262.00,552.92)(4.739,-0.495){35}{\rule{3.826pt}{0.119pt}}
\multiput(1262.00,553.17)(169.058,-19.000){2}{\rule{1.913pt}{0.400pt}}
\put(1216.0,565.0){\usebox{\plotpoint}}
\put(60.0,40.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(1439.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60.0,860.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\end{picture}


==> xfig/profile-phase.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(60.0,40.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(1439.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60.0,860.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60,108){\usebox{\plotpoint}}
\put(613,107.67){\rule{1.204pt}{0.400pt}}
\multiput(613.00,107.17)(2.500,1.000){2}{\rule{0.602pt}{0.400pt}}
\put(60.0,108.0){\rule[-0.200pt]{133.218pt}{0.400pt}}
\put(619.17,109){\rule{0.400pt}{1.500pt}}
\multiput(618.17,109.00)(2.000,3.887){2}{\rule{0.400pt}{0.750pt}}
\put(618.0,109.0){\usebox{\plotpoint}}
\put(621,116){\usebox{\plotpoint}}
\put(621,116){\usebox{\plotpoint}}
\put(621.17,117){\rule{0.400pt}{3.300pt}}
\multiput(620.17,117.00)(2.000,9.151){2}{\rule{0.400pt}{1.650pt}}
\put(621.0,116.0){\usebox{\plotpoint}}
\put(622.67,154){\rule{0.400pt}{5.300pt}}
\multiput(622.17,154.00)(1.000,11.000){2}{\rule{0.400pt}{2.650pt}}
\put(623.0,133.0){\rule[-0.200pt]{0.400pt}{5.059pt}}
\put(623.67,199){\rule{0.400pt}{5.300pt}}
\multiput(623.17,199.00)(1.000,11.000){2}{\rule{0.400pt}{2.650pt}}
\put(624.0,176.0){\rule[-0.200pt]{0.400pt}{5.541pt}}
\put(624.67,292){\rule{0.400pt}{7.709pt}}
\multiput(624.17,292.00)(1.000,16.000){2}{\rule{0.400pt}{3.854pt}}
\put(625.0,221.0){\rule[-0.200pt]{0.400pt}{17.104pt}}
\put(625.67,397){\rule{0.400pt}{8.191pt}}
\multiput(625.17,397.00)(1.000,17.000){2}{\rule{0.400pt}{4.095pt}}
\put(626.0,324.0){\rule[-0.200pt]{0.400pt}{17.586pt}}
\put(626.67,530){\rule{0.400pt}{8.672pt}}
\multiput(626.17,530.00)(1.000,18.000){2}{\rule{0.400pt}{4.336pt}}
\put(627.0,431.0){\rule[-0.200pt]{0.400pt}{23.849pt}}
\put(627.67,660){\rule{0.400pt}{6.263pt}}
\multiput(627.17,660.00)(1.000,13.000){2}{\rule{0.400pt}{3.132pt}}
\put(628.0,566.0){\rule[-0.200pt]{0.400pt}{22.645pt}}
\put(628.67,723){\rule{0.400pt}{3.854pt}}
\multiput(628.17,723.00)(1.000,8.000){2}{\rule{0.400pt}{1.927pt}}
\put(629.0,686.0){\rule[-0.200pt]{0.400pt}{8.913pt}}
\put(630,739){\usebox{\plotpoint}}
\put(630,739){\usebox{\plotpoint}}
\put(629.67,758){\rule{0.400pt}{1.927pt}}
\multiput(629.17,758.00)(1.000,4.000){2}{\rule{0.400pt}{0.964pt}}
\put(630.0,739.0){\rule[-0.200pt]{0.400pt}{4.577pt}}
\put(630.67,777){\rule{0.400pt}{1.927pt}}
\multiput(630.17,777.00)(1.000,4.000){2}{\rule{0.400pt}{0.964pt}}
\put(631.0,766.0){\rule[-0.200pt]{0.400pt}{2.650pt}}
\put(632.17,787){\rule{0.400pt}{0.700pt}}
\multiput(631.17,787.00)(2.000,1.547){2}{\rule{0.400pt}{0.350pt}}
\put(632.0,785.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(634,790){\usebox{\plotpoint}}
\put(634,790.17){\rule{0.700pt}{0.400pt}}
\multiput(634.00,789.17)(1.547,2.000){2}{\rule{0.350pt}{0.400pt}}
\put(866,790.67){\rule{0.241pt}{0.400pt}}
\multiput(866.00,791.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(637.0,792.0){\rule[-0.200pt]{55.166pt}{0.400pt}}
\put(867.67,789){\rule{0.400pt}{0.482pt}}
\multiput(867.17,790.00)(1.000,-1.000){2}{\rule{0.400pt}{0.241pt}}
\put(869,787.67){\rule{0.241pt}{0.400pt}}
\multiput(869.00,788.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(867.0,791.0){\usebox{\plotpoint}}
\put(870,788){\usebox{\plotpoint}}
\put(869.67,779){\rule{0.400pt}{1.204pt}}
\multiput(869.17,781.50)(1.000,-2.500){2}{\rule{0.400pt}{0.602pt}}
\put(870.0,784.0){\rule[-0.200pt]{0.400pt}{0.964pt}}
\put(870.67,769){\rule{0.400pt}{1.927pt}}
\multiput(870.17,773.00)(1.000,-4.000){2}{\rule{0.400pt}{0.964pt}}
\put(871.0,777.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(871.67,733){\rule{0.400pt}{4.095pt}}
\multiput(871.17,741.50)(1.000,-8.500){2}{\rule{0.400pt}{2.048pt}}
\put(872.0,750.0){\rule[-0.200pt]{0.400pt}{4.577pt}}
\put(873,733){\usebox{\plotpoint}}
\put(872.67,689){\rule{0.400pt}{4.818pt}}
\multiput(872.17,699.00)(1.000,-10.000){2}{\rule{0.400pt}{2.409pt}}
\put(873.0,709.0){\rule[-0.200pt]{0.400pt}{5.782pt}}
\put(873.67,593){\rule{0.400pt}{6.263pt}}
\multiput(873.17,606.00)(1.000,-13.000){2}{\rule{0.400pt}{3.132pt}}
\put(874.0,619.0){\rule[-0.200pt]{0.400pt}{16.863pt}}
\put(874.67,479){\rule{0.400pt}{11.322pt}}
\multiput(874.17,502.50)(1.000,-23.500){2}{\rule{0.400pt}{5.661pt}}
\put(875.0,526.0){\rule[-0.200pt]{0.400pt}{16.140pt}}
\put(875.67,326){\rule{0.400pt}{7.468pt}}
\multiput(875.17,341.50)(1.000,-15.500){2}{\rule{0.400pt}{3.734pt}}
\put(876.0,357.0){\rule[-0.200pt]{0.400pt}{29.390pt}}
\put(876.67,238){\rule{0.400pt}{2.891pt}}
\multiput(876.17,244.00)(1.000,-6.000){2}{\rule{0.400pt}{1.445pt}}
\put(877.0,250.0){\rule[-0.200pt]{0.400pt}{18.308pt}}
\put(877.67,163){\rule{0.400pt}{4.095pt}}
\multiput(877.17,171.50)(1.000,-8.500){2}{\rule{0.400pt}{2.048pt}}
\put(878.0,180.0){\rule[-0.200pt]{0.400pt}{13.972pt}}
\put(878.67,134){\rule{0.400pt}{3.854pt}}
\multiput(878.17,142.00)(1.000,-8.000){2}{\rule{0.400pt}{1.927pt}}
\put(879.0,150.0){\rule[-0.200pt]{0.400pt}{3.132pt}}
\put(879.67,117){\rule{0.400pt}{2.650pt}}
\multiput(879.17,122.50)(1.000,-5.500){2}{\rule{0.400pt}{1.325pt}}
\put(880.0,128.0){\rule[-0.200pt]{0.400pt}{1.445pt}}
\put(881.17,111){\rule{0.400pt}{0.900pt}}
\multiput(880.17,113.13)(2.000,-2.132){2}{\rule{0.400pt}{0.450pt}}
\put(881.0,115.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(883.0,109.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(887,107.67){\rule{0.241pt}{0.400pt}}
\multiput(887.00,108.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(883.0,109.0){\rule[-0.200pt]{0.964pt}{0.400pt}}
\put(888.0,108.0){\rule[-0.200pt]{132.736pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(1439.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60.0,860.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\end{picture}


==> xfig/profile-velocity.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(60.0,40.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(1439.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60.0,860.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60,661){\usebox{\plotpoint}}
\multiput(60.00,661.58)(1.674,0.498){99}{\rule{1.433pt}{0.120pt}}
\multiput(60.00,660.17)(167.025,51.000){2}{\rule{0.717pt}{0.400pt}}
\multiput(230.00,712.61)(0.685,0.447){3}{\rule{0.633pt}{0.108pt}}
\multiput(230.00,711.17)(2.685,3.000){2}{\rule{0.317pt}{0.400pt}}
\multiput(234.00,715.58)(0.917,0.498){103}{\rule{0.832pt}{0.120pt}}
\multiput(234.00,714.17)(95.273,53.000){2}{\rule{0.416pt}{0.400pt}}
\multiput(331.00,768.58)(0.529,0.494){29}{\rule{0.525pt}{0.119pt}}
\multiput(331.00,767.17)(15.910,16.000){2}{\rule{0.263pt}{0.400pt}}
\multiput(348.00,784.60)(3.113,0.468){5}{\rule{2.300pt}{0.113pt}}
\multiput(348.00,783.17)(17.226,4.000){2}{\rule{1.150pt}{0.400pt}}
\multiput(370.00,788.59)(4.272,0.477){7}{\rule{3.220pt}{0.115pt}}
\multiput(370.00,787.17)(32.317,5.000){2}{\rule{1.610pt}{0.400pt}}
\put(409,792.67){\rule{4.336pt}{0.400pt}}
\multiput(409.00,792.17)(9.000,1.000){2}{\rule{2.168pt}{0.400pt}}
\multiput(427.58,791.45)(0.498,-0.643){81}{\rule{0.120pt}{0.614pt}}
\multiput(426.17,792.73)(42.000,-52.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(469.59,735.53)(0.489,-1.252){15}{\rule{0.118pt}{1.078pt}}
\multiput(468.17,737.76)(9.000,-19.763){2}{\rule{0.400pt}{0.539pt}}
\multiput(478.58,714.53)(0.498,-0.924){73}{\rule{0.120pt}{0.837pt}}
\multiput(477.17,716.26)(38.000,-68.263){2}{\rule{0.400pt}{0.418pt}}
\multiput(516.58,639.39)(0.494,-2.515){27}{\rule{0.119pt}{2.073pt}}
\multiput(515.17,643.70)(15.000,-69.697){2}{\rule{0.400pt}{1.037pt}}
\multiput(531.58,566.88)(0.497,-2.038){51}{\rule{0.120pt}{1.715pt}}
\multiput(530.17,570.44)(27.000,-105.441){2}{\rule{0.400pt}{0.857pt}}
\multiput(558.59,457.39)(0.489,-2.242){15}{\rule{0.118pt}{1.833pt}}
\multiput(557.17,461.19)(9.000,-35.195){2}{\rule{0.400pt}{0.917pt}}
\multiput(567.58,421.30)(0.495,-1.303){35}{\rule{0.119pt}{1.132pt}}
\multiput(566.17,423.65)(19.000,-46.651){2}{\rule{0.400pt}{0.566pt}}
\multiput(586.59,371.60)(0.485,-1.560){11}{\rule{0.117pt}{1.300pt}}
\multiput(585.17,374.30)(7.000,-18.302){2}{\rule{0.400pt}{0.650pt}}
\put(592.67,352){\rule{0.400pt}{0.964pt}}
\multiput(592.17,354.00)(1.000,-2.000){2}{\rule{0.400pt}{0.482pt}}
\put(594,350.17){\rule{0.900pt}{0.400pt}}
\multiput(594.00,351.17)(2.132,-2.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(598.58,345.05)(0.494,-1.386){27}{\rule{0.119pt}{1.193pt}}
\multiput(597.17,347.52)(15.000,-38.523){2}{\rule{0.400pt}{0.597pt}}
\multiput(613.59,306.59)(0.477,-0.599){7}{\rule{0.115pt}{0.580pt}}
\multiput(612.17,307.80)(5.000,-4.796){2}{\rule{0.400pt}{0.290pt}}
\put(618,301.67){\rule{0.241pt}{0.400pt}}
\multiput(618.00,302.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\put(619.17,297){\rule{0.400pt}{1.100pt}}
\multiput(618.17,299.72)(2.000,-2.717){2}{\rule{0.400pt}{0.550pt}}
\put(621.17,288){\rule{0.400pt}{1.700pt}}
\multiput(620.17,292.47)(2.000,-4.472){2}{\rule{0.400pt}{0.850pt}}
\put(621.0,296.0){\usebox{\plotpoint}}
\put(622.67,273){\rule{0.400pt}{1.927pt}}
\multiput(622.17,277.00)(1.000,-4.000){2}{\rule{0.400pt}{0.964pt}}
\put(623.0,281.0){\rule[-0.200pt]{0.400pt}{1.686pt}}
\put(623.67,258){\rule{0.400pt}{1.927pt}}
\multiput(623.17,262.00)(1.000,-4.000){2}{\rule{0.400pt}{0.964pt}}
\put(624.0,266.0){\rule[-0.200pt]{0.400pt}{1.686pt}}
\put(624.67,226){\rule{0.400pt}{2.409pt}}
\multiput(624.17,231.00)(1.000,-5.000){2}{\rule{0.400pt}{1.204pt}}
\put(625.0,236.0){\rule[-0.200pt]{0.400pt}{5.300pt}}
\put(625.67,194){\rule{0.400pt}{2.409pt}}
\multiput(625.17,199.00)(1.000,-5.000){2}{\rule{0.400pt}{1.204pt}}
\put(626.0,204.0){\rule[-0.200pt]{0.400pt}{5.300pt}}
\put(626.67,154){\rule{0.400pt}{2.650pt}}
\multiput(626.17,159.50)(1.000,-5.500){2}{\rule{0.400pt}{1.325pt}}
\put(627.0,165.0){\rule[-0.200pt]{0.400pt}{6.986pt}}
\put(627.67,119){\rule{0.400pt}{1.927pt}}
\multiput(627.17,123.00)(1.000,-4.000){2}{\rule{0.400pt}{0.964pt}}
\put(628.0,127.0){\rule[-0.200pt]{0.400pt}{6.504pt}}
\put(629,119){\usebox{\plotpoint}}
\put(628.67,104){\rule{0.400pt}{1.204pt}}
\multiput(628.17,106.50)(1.000,-2.500){2}{\rule{0.400pt}{0.602pt}}
\put(629.0,109.0){\rule[-0.200pt]{0.400pt}{2.409pt}}
\put(630,104){\usebox{\plotpoint}}
\put(630,104){\usebox{\plotpoint}}
\put(629.67,97){\rule{0.400pt}{0.482pt}}
\multiput(629.17,98.00)(1.000,-1.000){2}{\rule{0.400pt}{0.241pt}}
\put(630.0,99.0){\rule[-0.200pt]{0.400pt}{1.204pt}}
\put(630.67,92){\rule{0.400pt}{0.482pt}}
\multiput(630.17,93.00)(1.000,-1.000){2}{\rule{0.400pt}{0.241pt}}
\put(631.0,94.0){\rule[-0.200pt]{0.400pt}{0.723pt}}
\put(632,92){\usebox{\plotpoint}}
\put(632,90.67){\rule{0.482pt}{0.400pt}}
\multiput(632.00,91.17)(1.000,-1.000){2}{\rule{0.241pt}{0.400pt}}
\put(634,91){\usebox{\plotpoint}}
\put(637,89.67){\rule{1.204pt}{0.400pt}}
\multiput(637.00,90.17)(2.500,-1.000){2}{\rule{0.602pt}{0.400pt}}
\put(634.0,91.0){\rule[-0.200pt]{0.723pt}{0.400pt}}
\put(866,89.67){\rule{0.241pt}{0.400pt}}
\multiput(866.00,89.17)(0.500,1.000){2}{\rule{0.120pt}{0.400pt}}
\put(642.0,90.0){\rule[-0.200pt]{53.962pt}{0.400pt}}
\put(869,90.67){\rule{0.241pt}{0.400pt}}
\multiput(869.00,90.17)(0.500,1.000){2}{\rule{0.120pt}{0.400pt}}
\put(867.0,91.0){\rule[-0.200pt]{0.482pt}{0.400pt}}
\put(870,92){\usebox{\plotpoint}}
\put(870,92){\usebox{\plotpoint}}
\put(869.67,93){\rule{0.400pt}{0.482pt}}
\multiput(869.17,93.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\put(870.0,92.0){\usebox{\plotpoint}}
\put(871,95){\usebox{\plotpoint}}
\put(871,95){\usebox{\plotpoint}}
\put(870.67,95){\rule{0.400pt}{0.723pt}}
\multiput(870.17,95.00)(1.000,1.500){2}{\rule{0.400pt}{0.361pt}}
\put(872,98){\usebox{\plotpoint}}
\put(871.67,104){\rule{0.400pt}{1.204pt}}
\multiput(871.17,104.00)(1.000,2.500){2}{\rule{0.400pt}{0.602pt}}
\put(872.0,98.0){\rule[-0.200pt]{0.400pt}{1.445pt}}
\put(873,109){\usebox{\plotpoint}}
\put(872.67,116){\rule{0.400pt}{1.445pt}}
\multiput(872.17,116.00)(1.000,3.000){2}{\rule{0.400pt}{0.723pt}}
\put(873.0,109.0){\rule[-0.200pt]{0.400pt}{1.686pt}}
\put(873.67,144){\rule{0.400pt}{2.168pt}}
\multiput(873.17,144.00)(1.000,4.500){2}{\rule{0.400pt}{1.084pt}}
\put(874.0,122.0){\rule[-0.200pt]{0.400pt}{5.300pt}}
\put(874.67,174){\rule{0.400pt}{3.614pt}}
\multiput(874.17,174.00)(1.000,7.500){2}{\rule{0.400pt}{1.807pt}}
\put(875.0,153.0){\rule[-0.200pt]{0.400pt}{5.059pt}}
\put(875.67,228){\rule{0.400pt}{2.650pt}}
\multiput(875.17,228.00)(1.000,5.500){2}{\rule{0.400pt}{1.325pt}}
\put(876.0,189.0){\rule[-0.200pt]{0.400pt}{9.395pt}}
\put(876.67,264){\rule{0.400pt}{0.964pt}}
\multiput(876.17,264.00)(1.000,2.000){2}{\rule{0.400pt}{0.482pt}}
\put(877.0,239.0){\rule[-0.200pt]{0.400pt}{6.022pt}}
\put(877.67,288){\rule{0.400pt}{1.445pt}}
\multiput(877.17,288.00)(1.000,3.000){2}{\rule{0.400pt}{0.723pt}}
\put(878.0,268.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(878.67,300){\rule{0.400pt}{1.445pt}}
\multiput(878.17,300.00)(1.000,3.000){2}{\rule{0.400pt}{0.723pt}}
\put(879.0,294.0){\rule[-0.200pt]{0.400pt}{1.445pt}}
\put(879.67,309){\rule{0.400pt}{1.445pt}}
\multiput(879.17,309.00)(1.000,3.000){2}{\rule{0.400pt}{0.723pt}}
\put(880.0,306.0){\rule[-0.200pt]{0.400pt}{0.723pt}}
\put(881.17,317){\rule{0.400pt}{0.900pt}}
\multiput(880.17,317.00)(2.000,2.132){2}{\rule{0.400pt}{0.450pt}}
\put(881.0,315.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\multiput(883.60,323.00)(0.468,1.358){5}{\rule{0.113pt}{1.100pt}}
\multiput(882.17,323.00)(4.000,7.717){2}{\rule{0.400pt}{0.550pt}}
\put(886.67,333){\rule{0.400pt}{0.482pt}}
\multiput(886.17,333.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\put(887.67,335){\rule{0.400pt}{0.482pt}}
\multiput(887.17,335.00)(1.000,1.000){2}{\rule{0.400pt}{0.241pt}}
\multiput(889.58,337.00)(0.494,0.680){25}{\rule{0.119pt}{0.643pt}}
\multiput(888.17,337.00)(14.000,17.666){2}{\rule{0.400pt}{0.321pt}}
\multiput(903.58,356.00)(0.494,2.002){27}{\rule{0.119pt}{1.673pt}}
\multiput(902.17,356.00)(15.000,55.527){2}{\rule{0.400pt}{0.837pt}}
\multiput(918.58,415.00)(0.496,1.313){37}{\rule{0.119pt}{1.140pt}}
\multiput(917.17,415.00)(20.000,49.634){2}{\rule{0.400pt}{0.570pt}}
\multiput(938.58,467.00)(0.494,2.627){25}{\rule{0.119pt}{2.157pt}}
\multiput(937.17,467.00)(14.000,67.523){2}{\rule{0.400pt}{1.079pt}}
\multiput(952.58,539.00)(0.498,1.606){79}{\rule{0.120pt}{1.378pt}}
\multiput(951.17,539.00)(41.000,128.140){2}{\rule{0.400pt}{0.689pt}}
\multiput(993.59,670.00)(0.488,1.154){13}{\rule{0.117pt}{1.000pt}}
\multiput(992.17,670.00)(8.000,15.924){2}{\rule{0.400pt}{0.500pt}}
\multiput(1001.58,688.00)(0.498,1.394){77}{\rule{0.120pt}{1.210pt}}
\multiput(1000.17,688.00)(40.000,108.489){2}{\rule{0.400pt}{0.605pt}}
\multiput(1041.00,797.92)(1.769,-0.492){19}{\rule{1.482pt}{0.118pt}}
\multiput(1041.00,798.17)(34.924,-11.000){2}{\rule{0.741pt}{0.400pt}}
\multiput(1079.00,788.60)(0.774,0.468){5}{\rule{0.700pt}{0.113pt}}
\multiput(1079.00,787.17)(4.547,4.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(1085.00,790.92)(2.320,-0.491){17}{\rule{1.900pt}{0.118pt}}
\multiput(1085.00,791.17)(41.056,-10.000){2}{\rule{0.950pt}{0.400pt}}
\multiput(1130.00,780.93)(0.492,-0.485){11}{\rule{0.500pt}{0.117pt}}
\multiput(1130.00,781.17)(5.962,-7.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(1137.00,773.92)(0.842,-0.498){91}{\rule{0.772pt}{0.120pt}}
\multiput(1137.00,774.17)(77.397,-47.000){2}{\rule{0.386pt}{0.400pt}}
\put(1216,726.67){\rule{0.241pt}{0.400pt}}
\multiput(1216.00,727.17)(0.500,-1.000){2}{\rule{0.120pt}{0.400pt}}
\multiput(1217.00,725.95)(1.579,-0.447){3}{\rule{1.167pt}{0.108pt}}
\multiput(1217.00,726.17)(5.579,-3.000){2}{\rule{0.583pt}{0.400pt}}
\multiput(1225.00,722.92)(1.250,-0.494){27}{\rule{1.087pt}{0.119pt}}
\multiput(1225.00,723.17)(34.745,-15.000){2}{\rule{0.543pt}{0.400pt}}
\multiput(1262.00,707.92)(1.366,-0.499){127}{\rule{1.189pt}{0.120pt}}
\multiput(1262.00,708.17)(174.532,-65.000){2}{\rule{0.595pt}{0.400pt}}
\put(883.0,321.0){\rule[-0.200pt]{0.400pt}{0.482pt}}
\put(60.0,40.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(1439.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\put(60.0,860.0){\rule[-0.200pt]{332.201pt}{0.400pt}}
\put(60.0,40.0){\rule[-0.200pt]{0.400pt}{197.538pt}}
\end{picture}

